Coordinating users of shared facilities via data-driven predictive assistants and game theory

We study data-driven assistants that provide congestion forecasts to users of shared facilities (roads, cafeterias, etc.), to support coordination between them, and increase efficiency of such collective systems. Key questions are: (1) when and how much can (accurate) predictions help for coordination, and (2) which assistant algorithms reach optimal predictions? First we lay conceptual ground for this setting where user preferences are a priori unknown and predictions influence outcomes. Addressing (1), we establish conditions under which self-fulfilling prophecies, i.e., "perfect" (probabilistic) predictions of what will happen, solve the coordination problem in the game-theoretic sense of selecting a Bayesian Nash equilibrium (BNE). Next we prove that such prophecies exist even in large-scale settings where only aggregated statistics about users are available. This entails a new (nonatomic) BNE existence result. Addressing (2), we propose two assistant algorithms that sequentially learn from users' reactions, together with optimality/convergence guarantees. We validate one of them in a large real-world experiment.

==> incl/raw_plots/eval.tex <==
% This file was created by matplotlib2tikz v0.6.14.
\begin{tikzpicture}

\definecolor{color2}{rgb}{0.319607843137255,0.279582592596744,0.989980213280707}
\definecolor{color0}{rgb}{0.5,0,1}
\definecolor{color1}{rgb}{0.413725490196078,0.135105247481393,0.997705180173873}

\begin{axis}[
xmin=-0.055, xmax=0.055,
ymin=-0.055, ymax=0.055,
width=\figwidth,
height=\figheight,
tick align=outside,
tick pos=left,
y grid style={lightgray!92.02614379084967!black},
legend entries={{Truth},{Average},{Expodamp}},
legend style={draw=white!80.0!black},
legend cell align={left}
]
\addlegendimage{no markers, color0}
\addlegendimage{no markers, color1}
\addlegendimage{no markers, color2}
\end{axis}

\node at ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$})[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{ };
\end{tikzpicture}
